Asynchronous Optimization Methods for Efficient Training of Deep Neural Networks with Guarantees

Asynchronous distributed algorithms are a popular way to reduce synchronization costs in large-scale optimization, and in particular for neural network training. However, for nonsmooth and nonconvex objectives, few convergence guarantees exist beyond cases where closed-form proximal operator solutions are available. As most popular contemporary deep neural networks lead to nonsmooth and nonconvex objectives, there is now a pressing need for such convergence guarantees. In this paper, we analyze for the first time the convergence of stochastic asynchronous optimization for this general class of objectives. In particular, we focus on stochastic subgradient methods allowing for block variable partitioning, where the shared-memory-based model is asynchronously updated by concurrent processes. To this end, we first introduce a probabilistic model which captures key features of real asynchronous scheduling between concurrent processes; under this model, we establish convergence with probability one to an invariant set for stochastic subgradient methods with momentum. From the practical perspective, one issue with the family of methods we consider is that it is not efficiently supported by machine learning frameworks, as they mostly focus on distributed data-parallel strategies. To address this, we propose a new implementation strategy for shared-memory based training of deep neural networks, whereby concurrent parameter servers are utilized to train a partitioned but shared model in single- and multi-GPU settings. Based on this implementation, we achieve on average 1.2x speed-up in comparison to state-of-the-art training methods for popular image classification tasks without compromising accuracy.

==> results/res20cifar10/pdf_plots/Arch_res20_Data_cifar10.tex <==
\begin{tabular}{p{0mm}p{16mm}p{3.5mm}p{3.5mm}p{3.5mm}p{3.5mm}p{3.5mm}}
\toprule\scriptsize
{} & Algo & Train{\newline}Loss & Train{\newline}Acc@1 & Test{\newline}Loss & Test{\newline}Acc@1 & Time{\newline}(Sec) \\
\midrule
(1) &          ASSM &     0.011 &      99.85 &    0.257 &     92.70 &     2102 \\
(2) &         PASSM &     0.097 &      96.83 &    0.302 &     91.03 &      992 \\
(3) &           Seq (BS=1024)&     0.008 &      99.94 &    0.245 &     92.57 &     1908 \\
(4) &           Seq &     0.011 &      99.88 &    0.234 &     93.07 &     2042 \\
(5) &       {PASSM$+$} &     {0.008} &     {100.00} &    0.246 &     \textbf{93.00} &     \textbf{1522} \\
\bottomrule
\end{tabular}


==> results/res20cifar10/result.tex <==
\begin{figure*}[t]
\centering
\adjustbox{valign=b}{\subfigure[Performance.]{%
\scriptsize\vspace{0pt}
\input{results/res20cifar10/pdf_plots/Arch_res20_Data_cifar10}
}}
\hfill
\adjustbox{valign=b}{\subfigure[Train Loss.]{%
\includegraphics[width=0.25\textwidth]{results/res20cifar10/pdf_plots/epTrainLoss}
}}
\hfill
\adjustbox{valign=b}{\subfigure[Top1 Test Accuracy.]{%
	\includegraphics[width=0.25\textwidth]{results/res20cifar10/pdf_plots/epTestAcc_1}
}}\caption{\small Resnet20/CIFAR10 training over a single Nvidia GeForce RTX 2080 Ti: Each of the runs use a mini-batch size 256, except the large batch one (BS=1024), where we do LR warm-up \cite{goyal2017accurate}. Async. methods train with 4 concurrent processes. Learning rate, weight-decay, momentum are identical to those in \cite{he2016deep}. }\label{fig:rn20-cifar10}
\end{figure*}

==> results/res20cifar100/pdf_plots/Arch_res20_Data_cifar100.tex <==
\begin{tabular}{p{0mm}p{16mm}p{3.5mm}p{3.5mm}p{3.5mm}p{3.5mm}p{3.5mm}}
	\toprule\scriptsize
	{} & Algo & Train{\newline}Loss & Train{\newline}Acc@1 & Test{\newline}Loss & Test{\newline}Acc@1 & Time{\newline}(Sec) \\
	\midrule
(1) &          ASSM &     0.289 &    92.71 &    1.125 &       68.89 &     1808 \\
(2) &         PASSM &     3.805 &    21.66 &     3.806 &      21.52 &     1257 \\
(3) &       P\_PASSM &     0.285 &    91.83 &     1.136 &      68.79 &     1523 \\
(4) &           Seq (BS=1024)&     0.258 &    93.53 &     1.143 &      68.51 &     1747 \\
(5) &           Seq &     0.303 &    92.02 &     1.107 &      69.02 &     1999 \\
\bottomrule
\end{tabular}


==> results/res20cifar100/result.tex <==
\begin{figure*}[t]
\centering
\adjustbox{valign=b}{\subfigure[Performance.]{%
\scriptsize\vspace{0pt}
\input{results/res20cifar100/pdf_plots/Arch_res20_Data_cifar100}
}}
\hfill
\adjustbox{valign=b}{\subfigure[Train Loss.]{%
\includegraphics[width=0.25\textwidth]{results/res20cifar100/pdf_plots/epTrainLoss}
}}
\hfill
\adjustbox{valign=b}{\subfigure[Top1 Test Accuracy.]{%
	\includegraphics[width=0.25\textwidth]{results/res20cifar100/pdf_plots/epTestAcc_1}
}}
\end{figure*}

==> sys.tex <==
\paragraph{Asynchronous System Specification.} 
We consider a shared-memory system with $p$ processes concurrently and asynchronously performing computations on independent compute-cores. We interchangeably use the terms process and core. The memory allows concurrent-read-concurrent-write (CRCW)\footnote{The proposed method will work even if only a CREW access is available because of partitioning of variables.} access. The shared-memory system offers word-sized atomic \texttt{read} and \texttt{fetch-and-add (faa)} primitives. Processes use \texttt{faa} to update the components of the variable.
